A Journey across the Hertzsprung-Russell diagram with 3D hydrodynamical simulations of cool stars

In this manuscript I summarise the work I have carried out in the last 10 years. My research projects are articulated around various fields in astrophysics having, as unifying theme, the 3D modelling and the observation of stellar atmospheres. In particular, my field of research covers all late type stars, from the Main Sequence stars to the advanced stages (red giant and supergiant stars). My work is based on the quantitative analysis of images, synthetic spectra, bolometric luminosity, planetary transits of different types of stars and on the modeling of their atmospheres. They include the use and development of 3D simunlations that are necessary for the interpretation of the data obtained with the new instruments equipping the space borne and ground telescopes. Interferometry and spectroscopy hold a privileged place in my research. My research themes concern interdisciplinary aspects by addressing questions related to atmospheric physics in relation to 3D hydrodynamic models. The predictions thus obtained are used to drive a vast campaign of interferometric, astrometric, photometric, spectroscopic and imaging observations. Finally, 3D simulations are also directly used to drive the development of new generation instrument at the VLTI, as well as very large future observatories and are directly linked to the ESA Gaia and PLATO missions.

==> abstract.tex <==
%auto-ignore 
% !TEX root = main.tex
%
% This section is the thesis abstract in English.
%
\prefacesection{Abstract}

\vspace{-1.0cm}
The study of primitive asteroids has gained much momentum in the last decade. 
The term \emph{primitive asteroid} usually refers to objects with low visible albedos ($\la$10\%) and mostly featureless visible-to-near-infrared spectra with  slopes ranging from slightly negative to moderately positive. %  (in other words, objects that fall within the so-called spectroscopic C-complex). 
These spectral characteristics are similar to those of the carbonaceous chondrites, the most primitive meteorites, some of which have been found to contain material predating the formation of the Solar System. 
Therefore, the study of primitive asteroids can reveal information about the origin and evolution of our planetary system since its early stages. 




